Better Understanding Differences in Attribution Methods via Systematic Evaluations

Deep neural networks are very successful on many vision tasks, but hard to interpret due to their black box nature. To overcome this, various post-hoc attribution methods have been proposed to identify image regions most influential to the models' decisions. Evaluating such methods is challenging since no ground truth attributions exist. We thus propose three novel evaluation schemes to more reliably measure the faithfulness of those methods, to make comparisons between them more fair, and to make visual inspection more systematic. To address faithfulness, we propose a novel evaluation setting (DiFull) in which we carefully control which parts of the input can influence the output in order to distinguish possible from impossible attributions. To address fairness, we note that different methods are applied at different layers, which skews any comparison, and so evaluate all methods on the same layers (ML-Att) and discuss how this impacts their performance on quantitative metrics. For more systematic visualizations, we propose a scheme (AggAtt) to qualitatively evaluate the methods on complete datasets. We use these evaluation schemes to study strengths and shortcomings of some widely used attribution methods over a wide range of models. Finally, we propose a post-processing smoothing step that significantly improves the performance of some attribution methods, and discuss its applicability.

==> commands.tex <==
\usepackage{xcolor}
\usepackage{etoolbox}
\usepackage[export]{adjustbox}
\usepackage{caption}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{e.g\onedot} \def\Eg{E.g\onedot}
\def\ie{i.e\onedot} \def\Ie{I.e\onedot}
\def\dh{d.h\onedot} \def\Dh{D.h\onedot}
\def\cf{cf\onedot} \def\Cf{Cf\onedot}
\def\etc{etc\onedot} \def\vs{vs\onedot}
\def\bzw{bzw\onedot}
\def\st{s.t\onedot}
\def\wrt{wrt\onedot}
\def\dof{d.o.f\onedot}
\def\etal{et~al\onedot} \def\iid{i.i.d\onedot}
\def\Fig{Fig\onedot} \def\Eqn{Eqn\onedot} \def\Sec{Sec\onedot} \def\Alg{Alg\onedot}
\makeatother

\newcommand{\pg}{GridPG\xspace}
\newcommand{\disc}{DiFull\xspace}
\newcommand{\cs}{DiPart\xspace}
\newcommand{\aggatt}{AggAtt\xspace}
\newcommand{\mlatt}{ML-Att\xspace}

% Helpful synonyms
\newcommand{\gridpg}{\pg}
\newcommand{\difull}{\disc}
\newcommand{\dipart}{\cs} 

\newcommand{\gb}{Guided Backprop\xspace}
\newcommand{\grad}{Gradient\xspace}
\newcommand{\intgrad}{IntGrad\xspace}
\newcommand{\sintgrad}{S-IntGrad\xspace}
\newcommand{\ixg}{IxG\xspace}
\newcommand{\sixg}{S-IxG\xspace}
\newcommand{\fullgrad}{FullGrad\xspace}
\newcommand{\smoothgrad}{SmoothGrad\xspace}
\newcommand{\gradcam}{Grad-CAM\xspace}
\newcommand{\gradcampp}{Grad-CAM++\xspace}
\newcommand{\scorecam}{Score-CAM\xspace}
\newcommand{\ablationcam}{Ablation-CAM\xspace}
\newcommand{\layercam}{Layer-CAM\xspace}
\newcommand{\cam}{CAM\xspace}
\newcommand{\detgradcam}{DetGrad-CAM\xspace}
\newcommand{\occ}{Occlusion\xspace}
\newcommand{\rise}{RISE\xspace}


% some space savers
\newcommand{\rulesep}{\unskip\ \vrule\ }
\newcommand\myeq{\mkern1.25mu{=}\mkern1.25mu}
\newcommand\mytimes{\mkern1.25mu{\times}\mkern1.25mu}
\setlength{\abovedisplayskip}{.25em}
\setlength{\belowdisplayskip}{.25em}
\setlength{\abovedisplayshortskip}{.25em}
\setlength{\belowdisplayshortskip}{.25em}
\setlength{\abovecaptionskip}{.25em}
\setlength{\belowcaptionskip}{.25em}
\setlength{\floatsep}{.25em}
\setlength{\textfloatsep}{.25em}
\newcommand\mysubsub[1]{\vspace{-.7em}%
\subsubsection{#1}%
\vspace{-.6em}
}

\newcommand{\myparagraph}[2][-.1]{\vspace{#1em}\noindent{\bf #2}}

\usepackage{float}
\usepackage{tabularx}
\usepackage{multirow}


==> table_correlation_vgg11.tex <==
\begin{figure}[H]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{} & Gradient & G. Backprop & IntGrad & IxG & Grad-CAM & Grad-CAM++ & Abl.-CAM & Score-CAM & Layer-CAM & Occlusion & RISE \\
\hline
\hline
\multirow{3}{*}{Gradient} & Inp & & 0.64 & 0.69 & 0.71 & -0.08 & 0.00 & -0.11 & -0.13 & 0.19 & 0.40 & 0.24 \\
& Mid & & 0.87 & 0.71 & 0.73 & 0.13 & -0.09 & 0.08 & -0.07 & 0.82 & 0.58 & 0.23 \\
& Fin & & 0.89 & 0.49 & 0.50 & 0.39 & 0.14 & 0.31 & 0.07 & 0.40 & 0.47 & 0.41 \\
\hline
\multirow{3}{*}{G. Backprop} & Inp & 0.64 & & 0.50 & 0.37 & -0.05 & -0.14 & -0.05 & -0.15 & 0.11 & 0.34 & 0.34 \\
& Mid & 0.87 & & 0.75 & 0.76 & 0.08 & 0.00 & 0.00 & 0.00 & 0.81 & 0.61 & 0.19 \\
& Fin & 0.89 & & 0.53 & 0.55 & 0.43 & 0.10 & 0.31 & 0.00 & 0.35 & 0.58 & 0.61 \\
\hline
\multirow{3}{*}{IntGrad} & Inp & 0.69 & 0.50 & & 0.94 & 0.00 & 0.25 & 0.12 & 0.09 & 0.29 & 0.43 & 0.20 \\
& Mid & 0.71 & 0.75 & & 0.98 & 0.14 & 0.24 & 0.29 & 0.30 & 0.88 & 0.76 & 0.41 \\
& Fin & 0.49 & 0.53 & & 0.99 & 0.87 & 0.68 & 0.79 & 0.54 & 0.87 & 0.86 & 0.65 \\
\hline
\multirow{3}{*}{IxG} & Inp & 0.71 & 0.37 & 0.94 & & 0.00 & 0.30 & 0.10 & 0.09 & 0.28 & 0.42 & 0.13 \\
& Mid & 0.73 & 0.76 & 0.98 & & 0.14 & 0.25 & 0.30 & 0.28 & 0.90 & 0.79 & 0.41 \\
& Fin & 0.50 & 0.55 & 0.99 & & 0.87 & 0.67 & 0.78 & 0.51 & 0.85 & 0.89 & 0.71 \\
\hline
\multirow{3}{*}{Grad-CAM} & Inp & -0.08 & -0.05 & 0.00 & 0.00 & & 0.05 & 0.13 & 0.18 & 0.11 & 0.00 & 0.00 \\
& Mid & 0.13 & 0.08 & 0.14 & 0.14 & & 0.19 & 0.57 & 0.24 & 0.14 & 0.00 & 0.05 \\
& Fin & 0.39 & 0.43 & 0.87 & 0.87 & & 0.73 & 0.85 & 0.57 & 0.74 & 0.78 & 0.63 \\
\hline
\multirow{3}{*}{Grad-CAM++} & Inp & 0.00 & -0.14 & 0.25 & 0.30 & 0.05 & & 0.09 & 0.15 & 0.07 & 0.09 & -0.07 \\
& Mid & -0.09 & 0.00 & 0.24 & 0.25 & 0.19 & & 0.46 & 0.77 & 0.36 & 0.08 & -0.05 \\
& Fin & 0.14 & 0.10 & 0.68 & 0.67 & 0.73 & & 0.70 & 0.69 & 0.85 & 0.48 & 0.29 \\
\hline
\multirow{3}{*}{Abl.-CAM} & Inp & -0.11 & -0.05 & 0.12 & 0.10 & 0.13 & 0.09 & & 0.65 & 0.55 & 0.05 & -0.06 \\
& Mid & 0.08 & 0.00 & 0.29 & 0.30 & 0.57 & 0.46 & & 0.50 & 0.26 & 0.16 & 0.23 \\
& Fin & 0.31 & 0.31 & 0.79 & 0.78 & 0.85 & 0.70 & & 0.64 & 0.73 & 0.66 & 0.50 \\
\hline
\multirow{3}{*}{Score-CAM} & Inp & -0.13 & -0.15 & 0.09 & 0.09 & 0.18 & 0.15 & 0.65 & & 0.77 & 0.07 & -0.10 \\
& Mid & -0.07 & 0.00 & 0.30 & 0.28 & 0.24 & 0.77 & 0.50 & & 0.31 & 0.07 & 0.05 \\
& Fin & 0.07 & 0.00 & 0.54 & 0.51 & 0.57 & 0.69 & 0.64 & & 0.65 & 0.30 & 0.16 \\
\hline
\multirow{3}{*}{Layer-CAM} & Inp & 0.19 & 0.11 & 0.29 & 0.28 & 0.11 & 0.07 & 0.55 & 0.77 & & 0.21 & 0.00 \\
& Mid & 0.82 & 0.81 & 0.88 & 0.90 & 0.14 & 0.36 & 0.26 & 0.31 & & 0.67 & 0.23 \\
& Fin & 0.40 & 0.35 & 0.87 & 0.85 & 0.74 & 0.85 & 0.73 & 0.65 & & 0.64 & 0.40 \\
\hline
\multirow{3}{*}{Occlusion} & Inp & 0.40 & 0.34 & 0.43 & 0.42 & 0.00 & 0.09 & 0.05 & 0.07 & 0.21 & & 0.21 \\
& Mid & 0.58 & 0.61 & 0.76 & 0.79 & 0.00 & 0.08 & 0.16 & 0.07 & 0.67 & & 0.32 \\
& Fin & 0.47 & 0.58 & 0.86 & 0.89 & 0.78 & 0.48 & 0.66 & 0.30 & 0.64 & & 0.82 \\
\hline
\multirow{3}{*}{RISE} & Inp & 0.24 & 0.34 & 0.20 & 0.13 & 0.00 & -0.07 & -0.06 & -0.10 & 0.00 & 0.21 & \\
& Mid & 0.23 & 0.19 & 0.41 & 0.41 & 0.05 & -0.05 & 0.23 & 0.05 & 0.23 & 0.32 & \\
& Fin & 0.41 & 0.61 & 0.65 & 0.71 & 0.63 & 0.29 & 0.50 & 0.16 & 0.40 & 0.82 & \\
\hline
\end{tabular}
}
\captionof{table}{\textbf{Spearman rank correlation coefficients between each pair of attribution methods at the input, middle, and final layers on \gridpg using VGG11.} All correlation coefficients are computed at identical layers for each pair of methods. We observe that correlation between methods tends to increase at the final layer. For example, \gradcam is correlated with \intgrad, and \ixg at the final layer with a coefficient $0.87$, while it is $0.00$ at the input layer. Correlation coefficients where $p > 0.05$ have been reported as $0.00$.}
\label{tab:corr:vgg11}
\end{figure}
\begin{figure}[H]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{} & Gradient & G. Backprop & IntGrad & IxG & Grad-CAM & Grad-CAM++ & Abl.-CAM & Score-CAM & Layer-CAM & Occlusion & RISE \\
\hline
\hline
\multirow{3}{*}{Gradient} & Inp & & -0.05 & 0.58 & 0.69 & -0.09 & 0.06 & -0.09 & -0.07 & 0.20 & 0.40 & 0.00 \\
& Mid & & 0.37 & 0.44 & 0.63 & 0.00 & 0.21 & 0.06 & 0.11 & 0.92 & 0.40 & 0.00 \\
& Fin & & - & - & - & - & - & - & - & - & - & - \\
\hline
\multirow{3}{*}{G. Backprop} & Inp & -0.05 & & 0.06 & -0.06 & 0.00 & -0.10 & 0.00 & -0.10 & -0.07 & -0.17 & 0.24 \\
& Mid & 0.37 & & 0.34 & 0.19 & -0.17 & 0.12 & -0.18 & 0.00 & 0.37 & 0.18 & 0.12 \\
& Fin & - & & - & - & - & - & - & - & - & - & - \\
\hline
\multirow{3}{*}{IntGrad} & Inp & 0.58 & 0.06 & & 0.94 & 0.00 & 0.36 & 0.18 & 0.21 & 0.32 & 0.36 & 0.00 \\
& Mid & 0.44 & 0.34 & & 0.35 & 0.07 & 0.23 & 0.16 & 0.29 & 0.48 & 0.31 & 0.15 \\
& Fin & - & - & & 1.00 & 1.00 & 0.57 & 0.92 & 0.60 & 0.57 & 0.96 & 0.89 \\
\hline
\multirow{3}{*}{IxG} & Inp & 0.69 & -0.06 & 0.94 & & 0.00 & 0.37 & 0.14 & 0.19 & 0.34 & 0.39 & 0.00 \\
& Mid & 0.63 & 0.19 & 0.35 & & 0.13 & 0.27 & 0.12 & 0.16 & 0.75 & 0.58 & -0.07 \\
& Fin & - & - & 1.00 & & 1.00 & 0.57 & 0.92 & 0.60 & 0.57 & 0.96 & 0.89 \\
\hline
\multirow{3}{*}{Grad-CAM} & Inp & -0.09 & 0.00 & 0.00 & 0.00 & & 0.00 & 0.12 & 0.19 & 0.14 & 0.00 & 0.00 \\
& Mid & 0.00 & -0.17 & 0.07 & 0.13 & & 0.25 & 0.68 & 0.24 & 0.09 & 0.08 & 0.00 \\
& Fin & - & - & 1.00 & 1.00 & & 0.58 & 0.92 & 0.61 & 0.58 & 0.95 & 0.89 \\
\hline
\multirow{3}{*}{Grad-CAM++} & Inp & 0.06 & -0.10 & 0.36 & 0.37 & 0.00 & & 0.08 & 0.11 & 0.08 & 0.15 & -0.06 \\
& Mid & 0.21 & 0.12 & 0.23 & 0.27 & 0.25 & & 0.30 & 0.65 & 0.49 & 0.00 & 0.00 \\
& Fin & - & - & 0.57 & 0.57 & 0.58 & & 0.55 & 0.74 & 1.00 & 0.46 & 0.40 \\
\hline
\multirow{3}{*}{Abl.-CAM} & Inp & -0.09 & 0.00 & 0.18 & 0.14 & 0.12 & 0.08 & & 0.66 & 0.61 & 0.00 & 0.00 \\
& Mid & 0.06 & -0.18 & 0.16 & 0.12 & 0.68 & 0.30 & & 0.40 & 0.13 & 0.10 & 0.00 \\
& Fin & - & - & 0.92 & 0.92 & 0.92 & 0.55 & & 0.62 & 0.57 & 0.88 & 0.86 \\
\hline
\multirow{3}{*}{Score-CAM} & Inp & -0.07 & -0.10 & 0.21 & 0.19 & 0.19 & 0.11 & 0.66 & & 0.85 & 0.11 & -0.09 \\
& Mid & 0.11 & 0.00 & 0.29 & 0.16 & 0.24 & 0.65 & 0.40 & & 0.31 & -0.05 & 0.00 \\
& Fin & - & - & 0.60 & 0.60 & 0.61 & 0.74 & 0.62 & & 0.75 & 0.50 & 0.45 \\
\hline
\multirow{3}{*}{Layer-CAM} & Inp & 0.20 & -0.07 & 0.32 & 0.34 & 0.14 & 0.08 & 0.61 & 0.85 & & 0.18 & -0.09 \\
& Mid & 0.92 & 0.37 & 0.48 & 0.75 & 0.09 & 0.49 & 0.13 & 0.31 & & 0.42 & 0.00 \\
& Fin & - & - & 0.57 & 0.57 & 0.58 & 1.00 & 0.57 & 0.75 & & 0.46 & 0.39 \\
\hline
\multirow{3}{*}{Occlusion} & Inp & 0.40 & -0.17 & 0.36 & 0.39 & 0.00 & 0.15 & 0.00 & 0.11 & 0.18 & & 0.00 \\
& Mid & 0.40 & 0.18 & 0.31 & 0.58 & 0.08 & 0.00 & 0.10 & -0.05 & 0.42 & & -0.06 \\
& Fin & - & - & 0.96 & 0.96 & 0.95 & 0.46 & 0.88 & 0.50 & 0.46 & & 0.92 \\
\hline
\multirow{3}{*}{RISE} & Inp & 0.00 & 0.24 & 0.00 & 0.00 & 0.00 & -0.06 & 0.00 & -0.09 & -0.09 & 0.00 & \\
& Mid & 0.00 & 0.12 & 0.15 & -0.07 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -0.06 & \\
& Fin & - & - & 0.89 & 0.89 & 0.89 & 0.40 & 0.86 & 0.45 & 0.39 & 0.92 & \\
\hline
\end{tabular}
}
\captionof{table}{\textbf{Spearman rank correlation coefficients between each pair of attribution methods at the input, middle, and final layers on \gridpg using Resnet18.} All correlation coefficients are computed at identical layers for each pair of methods. We observe that correlation between methods tends to increase at the final layer. For example, \gradcam is correlated with \intgrad, and \ixg at the final layer with a coefficient $1.00$, while it is $0.00$ at the input layer. Correlation coefficients where $p > 0.05$ have been reported as $0.00$.}
\label{tab:corr:resnet18}
\end{figure}

